Bootstrap your own latent: A new approach to self-supervised Learning

We introduce Bootstrap Your Own Latent (BYOL), a new approach to self-supervised image representation learning. BYOL relies on two neural networks, referred to as online and target networks, that interact and learn from each other. From an augmented view of an image, we train the online network to predict the target network representation of the same image under a different augmented view. At the same time, we update the target network with a slow-moving average of the online network. While state-of-the art methods rely on negative pairs, BYOL achieves a new state of the art without them. BYOL reaches $74.3\%$ top-1 classification accuracy on ImageNet using a linear evaluation with a ResNet-50 architecture and $79.6\%$ with a larger ResNet. We show that BYOL performs on par or better than the current state of the art on both transfer and semi-supervised benchmarks. Our implementation and pretrained models are given on GitHub.

==> tables/finetune_imagenet_table.tex <==
\vskip 1.05em
\begin{tabular}{l l |r r r r}
     \toprule 
          Method & Architecture & \multicolumn{2}{c}{Top-1 accuracy (\%)} & \multicolumn{2}{c}{Top-5 accuracy (\%)} \\
          & & Frac.\,$1\%$ & Frac.\,$10\%$ & Frac.\,$1\%$ & Frac.\,$10\%$ \\
          \midrule \hline
          Supervised baseline & ResNet-$50$ & & & $48.4$ & $80.4$ \\
          \midrule
          \multicolumn{4}{l}{\emph{Methods using other label propagation:}}\\
          Pseudo-label & ResNet-$50$ & & & $51.6$ & $82.4$\\
         VAT+Entropy Min. & ResNet-$50$ & & & $47.0$ & $83.4$\\
         UDA (w. RandAug) & ResNet-$50$ & & & - & $88.5$\\
         FixMatch (w. RandAug) & ResNet-$50$ & & & - & $89.1$\\
         S4L (Rot+VAT+En. M.) & ResNet-$50$ ($4\times$) & & & - & $91.2$\\
         \midrule
         \hline
         \multicolumn{4}{l}{\emph{Representation learning only:}}\\
         InstDisc & ResNet-$50$ & & & $39.2$ & $77.4$\\
         BigBiGAN \cite{BigBiGAN} & RevNet-$50$ ($4\times$) & & & $55.2$ & $78.8$ \\
         PIRL \cite{PIRL}  & ResNet-$50$ & & & $57.2$ & $83.8$\\
         \CPCC \cite{CPCv2}  & ResNet-$161$ & & & $77.9$ & $91.2$\\
         
         \simclr \cite{SimCLR}  & ResNet-$50$ & $48.3$ & $65.6$ & $75.5$ & $87.8$\\
         \algo (ours) & ResNet-$50$ & \cellcolor{pearDark!20} $\bf{53.3}$ & \cellcolor{pearDark!20} $\bf{68.4}$ &\cellcolor{pearDark!20} $\bf{78.2}$ & \cellcolor{pearDark!20} $\bf{88.8}$\\
         \simclr \cite{SimCLR}   & ResNet-$50$ ($2\times$) & $58.5$ & $71.7$ & $83.0$ & $91.2$\\
          \algo (ours) & ResNet-$50$ ($2\times$) &\cellcolor{pearDark!20} $\bf{62.0}$ & \cellcolor{pearDark!20} $\bf{72.4}$ &\cellcolor{pearDark!20} $\bf{84.2}$ & \cellcolor{pearDark!20} $90.9$\\
         \simclr \cite{SimCLR}  & ResNet-$50$ ($4\times$) & $63.0$ & $74.4$ & $85.8$ & $92.6$\\
         \algo (ours) & ResNet-$50$ ($4\times$) &\cellcolor{pearDark!20} ?& \cellcolor{pearDark!20} ? &\cellcolor{pearDark!20} ? &\cellcolor{pearDark!20} ?\\
         \algo (ours) & ResNet-$152$ ($3\times$) & $\bf{67.4}$ & $\bf{74.7}$ & $\bf{86.9}$ & $91.5$\\
         \bottomrule
\end{tabular}

==> tables/linear_classif_table.tex <==
\begin{tabular}[t]{l l r| r r}
    \toprule
         Method & Architecture & Param. &  Top-$1$ & Top-$5$ \\
         \midrule \hline
         Local Agg. & ResNet-$50$ & $24$M & $60.2$ & -\\
         \moco \cite{MOCO} & ResNet-$50$ & $24$M & $60.6$ & -\\
         \PIRL \cite{PIRL} & ResNet-$50$ & $24$M & $63.6$ & -\\
         \CPCC \cite{CPCv2}  & ResNet-$50$ & $24$M & $63.8$ & $85.3$\\
         \simclr \cite{SimCLR} & ResNet-$50$ & $24$M & $69.8$ & $89.0$\\
         \moco v2 \cite{MOCOv2} & ResNet-$50$ & $24$M & $71.1$ & -\\
         InfoMin Aug. \cite{Tian2020WhatMF} & ResNet-$50$ & $24$M & $73.0$ & $91.1$\\
         \algo (ours) & ResNet-$50$ & $24$M & $\cellcolor{pearDark!20}\bf{74.3}$ & $\cellcolor{pearDark!20}\bf{91.9}$\\
\end{tabular}

\begin{tabular}[t]{l l r| r r}
\midrule \hline 
Method & Architecture & Param. &  Top-$1$ & Top-$5$ \\
         Rotation \cite{gidaris2018unsupervised} & RevNet-$50$ ($4\times$) & $86$M & $55.4$ & -\\
         BigBiGAN \cite{BigBiGAN} & RevNet-$50$ ($4\times$) & $86$M & $61.3$ & $81.9$\\
         AMDIM \cite{AMDIM} & Custom-ResNet & $626$M & $68.1$ & -\\
         \CMC \cite{CMC} & ResNet-$50$ ($2\times$) & $188$M & $68.4$ & $88.2$\\
         \moco \cite{MOCO} & ResNet-$50$ ($4\times$) & $375$M & $68.6$ & -\\
         \CPCC \cite{CPCv2}  & ResNet-$161$ & $305$M & $71.5$ & $90.1$\\
         \simclr \cite{SimCLR}  & ResNet-$50$ ($2\times$) & $94$M & $74.4$ & $92.0$\\
         \algo (ours) & ResNet-$50$ ($2\times$) & $94$M & \cellcolor{pearDark!20} $77.4$ & \cellcolor{pearDark!20} $93.7$\\
         \simclr \cite{SimCLR}  & ResNet-$50$ ($4\times$) & $375$M & $76.8$ & $93.2$\\
         \algo (ours) & ResNet-$50$ ($4\times$) & $375$M & $\cellcolor{pearDark!20}78.8$ &\cellcolor{pearDark!20} $94.4$\\
         \algo (ours) & ResNet-$152$ ($3\times$) & $522$M & $\cellcolor{pearDark!20}\bf{79.5}$ &\cellcolor{pearDark!20} $\bf{94.7}$\\
         \bottomrule
    \end{tabular}

















%\begin{table}[h!]
%\hspace{-3em}
%\begin{subtable}{.4\linewidth}
%\scriptsize
%\begin{center}
%    \input{tables/linear_classif_table.tex}
%     \caption{Linear evaluation on ImageNet.}
%    \label{table:linear_classif}
%    \end{center}
%    \end{subtable}
%    \phantom{aaaaa}
%    \begin{subtable}{.4\linewidth}
%   \scriptsize
%    \begin{center}
%     \input{tables/finetune_imagenet_table.tex}
%     \caption{Training with few labels.}
%     \label{table:few_lables}
%     \end{center}
%\end{subtable}
%\caption{ImageNet results}
%\end{table}



\begin{tabular}[t]{l l r| r r}
    \toprule
         Method & Architecture & Param. &  Top-$1$ & Top-$5$ \\
         \midrule \hline
%         \multicolumn{5}{l}{\emph{Using ResNet-$50$ architecture:}}\\
         Local Agg. & ResNet-$50$ & $24$M & $60.2$ & -\\
         \moco \cite{MOCO} & ResNet-$50$ & $24$M & $60.6$ & -\\
         \PIRL \cite{PIRL} & ResNet-$50$ & $24$M & $63.6$ & -\\
         \CPCC \cite{CPCv2}  & ResNet-$50$ & $24$M & $63.8$ & $85.3$\\
         \simclr \cite{SimCLR} & ResNet-$50$ & $24$M & $69.8$ & $89.0$\\
         \moco v2 \cite{MOCOv2} & ResNet-$50$ & $24$M & $71.1$ & -\\
         InfoMin Aug. \cite{Tian2020WhatMF} & ResNet-$50$ & $24$M & $73.0$ & $91.1$\\
         \algo (ours) & ResNet-$50$ & $24$M & $\cellcolor{pearDark!20}\bf{74.5}$ & $\cellcolor{pearDark!20}\bf{91.9}$\\
         \hline
%         \multicolumn{5}{l}{\emph{Using other architectures:}}\\
             \hline
         Rotation \cite{gidaris2018unsupervised} & RevNet-$50$ ($4\times$) & $86$M & $55.4$ & -\\
         BigBiGAN \cite{BigBiGAN} & RevNet-$50$ ($4\times$) & $86$M & $61.3$ & $81.9$\\
         AMDIM \cite{AMDIM} & Custom-ResNet & $626$M & $68.1$ & -\\
         \CMC \cite{CMC} & ResNet-$50$ ($2\times$) & $188$M & $68.4$ & $88.2$\\
         \moco \cite{MOCO} & ResNet-$50$ ($4\times$) & $375$M & $68.6$ & -\\
         \CPCC \cite{CPCv2}  & ResNet-$161$ & $305$M & $71.5$ & $90.1$\\
         \simclr \cite{SimCLR}  & ResNet-$50$ ($2\times$) & $94$M & $74.4$ & $92.0$\\
         \algo (ours) & ResNet-$50$ ($2\times$) & $94$M & \cellcolor{pearDark!20} $77.4$ & \cellcolor{pearDark!20} $93.7$\\
         \simclr \cite{SimCLR}  & ResNet-$50$ ($4\times$) & $375$M & $76.8$ & $93.2$\\
         \algo (ours) & ResNet-$50$ ($4\times$) & $375$M & $\cellcolor{pearDark!20}78.8$ &\cellcolor{pearDark!20} $94.4$\\
         \algo (ours) & ResNet-$152$ ($3\times$) & $522$M & $\cellcolor{pearDark!20}\bf{79.5}$ &\cellcolor{pearDark!20} $\bf{94.7}$\\
         \bottomrule
    \end{tabular}

\begin{tabular}[t]{l l r| r r}
    \toprule
         Method & Architecture & Param. &  Top-$1$ & Top-$5$ \\
         \midrule \hline
%         \multicolumn{5}{l}{\emph{Using ResNet-$50$ architecture:}}\\
         Local Agg. & ResNet-$50$ & $24$M & $60.2$ & -\\
         \moco \cite{MOCO} & ResNet-$50$ & $24$M & $60.6$ & -\\
         \PIRL \cite{PIRL} & ResNet-$50$ & $24$M & $63.6$ & -\\
         \CPCC \cite{CPCv2}  & ResNet-$50$ & $24$M & $63.8$ & $85.3$\\
         \simclr \cite{SimCLR} & ResNet-$50$ & $24$M & $69.8$ & $89.0$\\
         \moco v2 \cite{MOCOv2} & ResNet-$50$ & $24$M & $71.1$ & -\\
         InfoMin Aug. \cite{Tian2020WhatMF} & ResNet-$50$ & $24$M & $73.0$ & $91.1$\\
         \algo (ours) & ResNet-$50$ & $24$M & $\cellcolor{pearDark!20}\bf{74.5}$ & $\cellcolor{pearDark!20}\bf{91.9}$\\
         \hline
%         \multicolumn{5}{l}{\emph{Using other architectures:}}\\
             \hline
         Rotation \cite{gidaris2018unsupervised} & RevNet-$50$ ($4\times$) & $86$M & $55.4$ & -\\
         BigBiGAN \cite{BigBiGAN} & RevNet-$50$ ($4\times$) & $86$M & $61.3$ & $81.9$\\
         AMDIM \cite{AMDIM} & Custom-ResNet & $626$M & $68.1$ & -\\
         \CMC \cite{CMC} & ResNet-$50$ ($2\times$) & $188$M & $68.4$ & $88.2$\\
         \moco \cite{MOCO} & ResNet-$50$ ($4\times$) & $375$M & $68.6$ & -\\
         \CPCC \cite{CPCv2}  & ResNet-$161$ & $305$M & $71.5$ & $90.1$\\
         \simclr \cite{SimCLR}  & ResNet-$50$ ($2\times$) & $94$M & $74.4$ & $92.0$\\
         \algo (ours) & ResNet-$50$ ($2\times$) & $94$M & \cellcolor{pearDark!20} $77.4$ & \cellcolor{pearDark!20} $93.7$\\
         \simclr \cite{SimCLR}  & ResNet-$50$ ($4\times$) & $375$M & $76.8$ & $93.2$\\
         \algo (ours) & ResNet-$50$ ($4\times$) & $375$M & $\cellcolor{pearDark!20}78.8$ &\cellcolor{pearDark!20} $94.4$\\
         \algo (ours) & ResNet-$152$ ($3\times$) & $522$M & $\cellcolor{pearDark!20}\bf{79.5}$ &\cellcolor{pearDark!20} $\bf{94.7}$\\
         \bottomrule
    \end{tabular}

==> tables/semi_supervised_table.tex <==
\begin{table}[h]
\begin{subtable}{.4\linewidth}
    \tiny
    \centering
    \begin{tabular}{l l | r}
     \toprule 
          Method & Architecture & {Top-5 $10\%$}\\
          \midrule \hline
          Supervised baseline & ResNet-$50$ & $80.4$ \\
          \midrule
          Pseudo-label & ResNet-$50$ & $82.4$\\
         VAT+Entropy Min. & ResNet-$50$ & $83.4$\\
         UDA (w. RandAug) & ResNet-$50$ & $88.5$\\
         FixMatch (w. RandAug) & ResNet-$50$ 4& $89.1$\\
         S4L (Rot+VAT+En. M.) & ResNet-$50$ ($4\times$) & $\bf{91.2}$\\
         \bottomrule
    \end{tabular}
    \caption{\label{table:few_labels_1}Methods using other label propagation}
\end{subtable}
\phantom{aaaaa}
\begin{subtable}{.45\linewidth}
    \tiny
    \centering
    \begin{tabular}{l l |r r r r}
    \toprule
         Method & Architecture & \multicolumn{2}{c}{Top-1} & \multicolumn{2}{c}{Top-5} \\
          & & $1\%$ & $10\%$ & $1\%$ & $10\%$ \\
         \midrule \hline
         InstDisc & ResNet-$50$ & - & - & $39.2$ & $77.4$\\
         BigBiGAN \cite{BigBiGAN} & RevNet-$50$ ($4\times$) & - & - & $55.2$ & $78.8$ \\
         PIRL \cite{PIRL}  & ResNet-$50$ & - & - & $57.2$ & $83.8$\\
         \CPCC \cite{CPCv2}  & ResNet-$161$ & - & - & $77.9$ & $91.2$\\
         
         \simclr \cite{SimCLR}  & ResNet-$50$ & $48.3$ & $65.6$ & $75.5$ & $87.8$\\
         \algo (ours) & ResNet-$50$ & \cellcolor{pearDark!20} $\bf{53.3}$ & \cellcolor{pearDark!20} $\bf{67.6}$ &\cellcolor{pearDark!20} $\bf{78.4}$ & \cellcolor{pearDark!20} $\bf{88.7}$\\
         \simclr \cite{SimCLR}   & ResNet-$50$ ($2\times$) & $58.5$ & $71.7$ & $83.0$ & $91.2$\\
          \algo (ours) & ResNet-$50$ ($2\times$) &\cellcolor{pearDark!20} $\bf{62.2}$ & \cellcolor{pearDark!20} $\bf{(72.4)}$ &\cellcolor{pearDark!20} $\bf{84.1}$ & \cellcolor{pearDark!20} $(90.9)$\\
         \simclr \cite{SimCLR}  & ResNet-$50$ ($4\times$) & $63.0$ & $74.4$ & $85.8$ & $92.6$\\
         \algo (ours) & ResNet-$50$ ($4\times$) &\cellcolor{pearDark!20} $69.1$& \cellcolor{pearDark!20} $74.6$ &\cellcolor{pearDark!20} $87.9$ &\cellcolor{pearDark!20} $91.5$\\
         \algo (ours) & ResNet-$152$ ($3\times$) & $\bf{68.4}$ & $\bf{(74.7)}$ & $\bf{86.4}$ & $(91.5)$\\
         \bottomrule
    \end{tabular}
\caption{\label{table:few_labels_2}Representation methods only}
\end{subtable}
    \caption{\label{table:few_labels}Semi-supervised training (with few labels) on ImageNet.}
\end{table}

==> tables/simclr_to_pbl_table.tex <==
\begin{tabular}{l c c c c}
\toprule
Method & Predictor & Target network & $\beta$ & Top-1  \\
\midrule
\algo   & \checkmark & \checkmark &  0 & $72.6$ \\
        & \checkmark & \checkmark & 1 & $70.8$ \\
        &            & \checkmark & 1 & $70.8$\\
\simclr &            &            & 1 & $69.2$\\
        & \checkmark &            & 1 & $69.0$\\
        & \checkmark &            & 0 & $0.3$  \\
        &            & \checkmark & 0 & $0.2$  \\
        &            &            & 0 & $0.1$   \\
\bottomrule
\end{tabular}



==> tables/transfer_table_from_places2.tex <==
\setlength\tabcolsep{4.3pt}
\hspace{-0.1cm}
\begin{tabular}{l c c c c c c}
\cmidrule[\heavyrulewidth]{1-7}
{\small Method} &  {\small Places365} & {\small ImageNet} & {\small Food101} & {\small CIFAR10} & {\small CIFAR100} & {\small Birdsnap} \\
\midrule
\algo-IN & $51.0$ & $74.3$ & $75.3$ & $91.3$ & $78.4$ & $57.3$\\ \midrule
\algo-PL & \cellcolor{pearDark!20}$\bf{53.2}$ & \cellcolor{pearDark!20}$\bf{58.5}$ & \cellcolor{pearDark!20}$\bf{64.7}$ & \cellcolor{pearDark!20}$\bf{84.5}$ & \cellcolor{pearDark!20}$\bf{66.1}$ & \cellcolor{pearDark!20}$\bf{28.8}$ \\
\simclr-PL & $53.0$ & $56.5$ & $61.7$ & $80.8$ & $61.1$ & $21.2$ \\
\bottomrule
\end{tabular}

\setlength\tabcolsep{5.3pt}
\hspace{-0.1cm}
\begin{tabular}{l c c c c c c c}
\cmidrule[\heavyrulewidth]{1-8}
{\small Method} & {\small SUN397}  & {\small Cars} & {\small Aircraft} & {\small DTD} & {\small Pets} & {\small Caltech-101} & {\small Flowers} \\
\midrule
\algo-IN & $62.6$ & $67.2$ & $60.6$ & $76.5$ & $90.4$ & $94.3$ & $96.1$ \\ \midrule
\algo-PL & \cellcolor{pearDark!20}$\bf{64.2}$ & \cellcolor{pearDark!20}$\bf{55.6}$ & \cellcolor{pearDark!20}$\bf{55.9}$ & \cellcolor{pearDark!20}$\bf{68.5}$ & \cellcolor{pearDark!20}$\bf{66.1}$ & \cellcolor{pearDark!20}$\bf{84.3}$ & \cellcolor{pearDark!20}$\bf{90.0}$ \\
\simclr-PL & $62.5$ & $40.1$ & $44.3$ & $64.3$ & $59.4$ & $77.1$ & $85.9$ \\
\bottomrule
\end{tabular}

==> tables/transfer_to_imagenet_table.tex <==
\begin{tabular}{l c c c c}
\toprule
& Places365 & YFCC-100m & JFT-300m & JFT-300m \\
\midrule
Training dataset & ? & ? & ? & ? \\
Training steps & ? & ? & ? & ?  \\
ImageNet top-1 & ? & ? & ? & ? \\
\bottomrule
\end{tabular}
